POLIPHONE: A Dataset for Smartphone Model Identification from Audio Recordings

When dealing with multimedia data, source attribution is a key challenge from a forensic perspective. This task aims to determine how a given content was captured, providing valuable insights for various applications, including legal proceedings and integrity investigations. The source attribution problem has been addressed in different domains, from identifying the camera model used to capture specific photographs to detecting the synthetic speech generator or microphone model used to create or record given audio tracks. Recent advancements in this area rely heavily on machine learning and data-driven techniques, which often outperform traditional signal processing-based methods. However, a drawback of these systems is their need for large volumes of training data, which must reflect the latest technological trends to produce accurate and reliable predictions. This presents a significant challenge, as the rapid pace of technological progress makes it difficult to maintain datasets that are up-to-date with real-world conditions. For instance, in the task of smartphone model identification from audio recordings, the available datasets are often outdated or acquired inconsistently, making it difficult to develop solutions that are valid beyond a research environment. In this paper we present POLIPHONE, a dataset for smartphone model identification from audio recordings. It includes data from 20 recent smartphones recorded in a controlled environment to ensure reproducibility and scalability for future research. The released tracks contain audio data from various domains (i.e., speech, music, environmental sounds), making the corpus versatile and applicable to a wide range of use cases. We also present numerous experiments to benchmark the proposed dataset using a state-of-the-art classifier for smartphone model identification from audio recordings.

==> 05_results_OLD.tex <==
\section{Recording Microphone Identification}
\label{sec:results}

In this section, we benchmark the released dataset on the recording microphone identification task. We do so by considering three different methods proposed in the literature for this specific task and testing them in various scenarios.
The goal of these experiments is to evaluate the contribution that POLIPHONE can give to the state-of-the-art.

The problem we consider is formally defined as follows.
Given a discrete-time input speech signal $x$ sampled with sampling frequency $f_\text{s}$, and a set of $I$ recording devices $y_i \in \{y_0, ..., y_{I-1}\}$, the goal of the task is to develop a classifier $\mathcal{C}$ able to predict which device $y_i$ has been used to record $x$.

We performed the experiments considering three different classifiers $\mathcal{C}$, presented in the literature for recording microphone identification. These were chosen to represent three distinct approaches to the same problem, providing a broad overview of the possible strategies that can be used.
The first baseline focuses on analyzing the \gls{bed} between recordings~\cite{luo_bed_2018}, the second employs a \gls{cnn} as a multiclass classifier~\cite{baldini_cnn_2019}, and the third uses \gls{gmm} to estimate the channel response~\cite{giganti2022speaker}.
We refer readers to the corresponding original publications for more details about each specific baseline.
{\color{red} [TODO: AGGIUNGI PIU DETTAGLI BASELINES]}
% ANTONIO's baselines
As a first experiment, we test the baselines on the clean speech recordings included in the POLIPHONE dataset.
We do so as this is the most considered scenario for the recording microphone identification task, and it is also the one in which the considered baselines were designed.
We consider the data as it is released in the dataset, with a sampling rate $f_\text{s}$ = \SI{44.1}{\kilo\hertz}.
We also repeat the same experiment using a downsampled version of the tracks with a sampling frequency $f_\text{s}$ = \SI{16}{\kilo\hertz}. This aims to examine the impact of a rate change on the classification performance and analyze whether this change significantly impacts the achieved results or not. 
This is a relevant aspect that has never been investigated since most of the datasets present in the literature are sampled at $f_\text{s}$ = \SI{16}{\kilo\hertz}, as shown in \cref{tab:dataset_sota}.
To perform this experiment we considered the same training and test sets for all the classifiers. In particular, {\color{red} [TODO: DETTAGLI SU TRAINING E TEST SETS]}.

\begin{enumerate}
    
    \item \textbf{EXPERIMENT 1}: TRAIN Clean speech - TEST Clean speech -> \cref{tab:baseline_scores}
    
    \item \textbf{EXPERIMENT 2}: TRAIN Clean speech - TEST Noise speech -> \cref{tab:baseline_scores}

    \item \textbf{EXPERIMENT 3}: TRAIN Clean speech - TEST Clean speech - Allena su subsets del dataset di training -> \cref{fig::baseline_scores}

    \item \textbf{EXPERIMENT 4}: TRAIN Music + Environment TEST Clean speech -> \cref{tab:baselines_music_env}

    \item \textbf{EXPERIMENT 5}: TRAIN Clean speech original - TEST Clean speech convolved -> \cref{tab:baselines_convolved}

    \item \textbf{EXPERIMENT 6}: TRAIN Clean speech convolved - TEST Clean speech original -> \cref{tab:baselines_convolved}

    \item \textbf{EXPERIMENT 7}: TRAIN Clean speech anechoic - TEST Clean speech office -> TEST DA FARE
    
    \item \textbf{EXPERIMENT 8, aka 3bis}: TRAIN Noisy speech - TEST Noisy speech - Allena su subsets del dataset di training ->
    
\end{enumerate}

\begin{table}[]
\centering
\caption{Accuracy values of the three considered baselines, trained and tested on clean and noisy speech at both \SI{44}{\kilo\hertz} and \SI{16}{\kilo\hertz} as sampling frequency.}
\label{tab:baseline_scores}
\begin{tabular}{ccccc}
\toprule
\multicolumn{1}{l}{} & \multicolumn{2}{c}{Clean speech}            & \multicolumn{2}{c}{Noisy speech}            \\
            & \SI{44}{\kilo\hertz} & \SI{16}{\kilo\hertz} & \SI{44}{\kilo\hertz} & \SI{16}{\kilo\hertz} \\ \midrule
CNN~\cite{baldini_cnn_2019} &           98.44 & 83.17 & 99.44 & 89.77 \\
BED~\cite{luo_bed_2018} &           81.03 & 68.89 & 59.68 & 56.35 \\
Channel resp.~\cite{giganti2022speaker} & 99.76 & 95.95 & 79.68 & 89.60 \\ \bottomrule
\end{tabular}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=.9\columnwidth]{figures/baselines_percentage.pdf}
    \caption{Accuracy values of the three considered baselines, trained on different percentages of the training set. We report the metrics for the experiments considering both \SI{44}{\kilo\hertz} and \SI{16}{\kilo\hertz} as sampling frequency.}
    \label{fig:baselines_percentage}
\end{figure}


\begin{table}[]
\centering
\caption{Accuracy values of two of the considered baselines, trained music and environmental sounds recordings and tested on clean speech. The results are shown considering both \SI{44}{\kilo\hertz} and \SI{16}{\kilo\hertz} as sampling frequency.}
\label{tab:baselines_music_env}
\begin{tabular}{ccc}
\toprule
& \SI{44}{\kilo\hertz} & \SI{16}{\kilo\hertz} \\ \midrule
CNN~\cite{baldini_cnn_2019}       & 95.89            & 74.08            \\
BED~\cite{luo_bed_2018}       & 71.36            & 94.68 \\ \bottomrule              
\end{tabular}
\end{table}


\begin{table}[]
\centering
\caption{Accuracy values of the three considered baselines, trained on recorded speech and tested on convolved data, and vice versa. The results are shown considering both \SI{44}{\kilo\hertz} and \SI{16}{\kilo\hertz} as sampling frequency.}
\label{tab:baselines_convolved}
\begin{tabular}{ccccc}
\toprule
\multicolumn{1}{l}{} & \multicolumn{2}{c}{Test convolved speech}            & \multicolumn{2}{c}{Test clean speech}            \\
            & \SI{44}{\kilo\hertz} & \SI{16}{\kilo\hertz} & \SI{44}{\kilo\hertz} & \SI{16}{\kilo\hertz} \\ \midrule
CNN~\cite{baldini_cnn_2019} &           75.92 & 73.12 & 82.04 & 72.77 \\
BED~\cite{luo_bed_2018} &           63.73 & 66.43 & 63.49 & 61.11 \\
Channel resp.~\cite{giganti2022speaker} & 57.70 & 75.71 & 65.16 & 67.38 \\ \bottomrule
\end{tabular}
\end{table}

==> 06_discussion.tex <==
\section{Discussion}
\label{sec:discussion}

In this section we discuss the possible applications of the presented dataset (device ID but also domain adaptation)

{\color{red} [TODO: questa sezione la teniamo o la togliamo?]}

==> 08_biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/agiganti.jpeg}}]{Antonio Giganti} was born in Assisi, Italy, in 1995. He received the M.Sc degree in Music and Acoustic Engineering from the Politecnico di Milano, Italy, in 2021. He is currently a Ph.D. student with the Image and Sound Processing Lab (ISPL) at the Department of Electronics, Information and Bioengineering (DEIB) of the Politecnico di Milano. His research activity focuses on signal processing for multimedia forensics applications.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/dleonzio.jpeg}}]{Daniele Ugo Leonzio} was born in Foggia, Italy, in 1997. He received the M.Sc degree in Music and Acoustic Engineering from the Politecnico di Milano, Italy, in 2021. He is currently a Ph.D. student with the Image and Sound Processing Lab (ISPL) at the Department of Electronics, Information and Bioengineering (DEIB) of the Politecnico di Milano. His research activity focuses on the study of multimedia signal processing techniques.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/dsalvi.png}}]{Davide Salvi} was born in Bergamo, Italy, in 1995. He received the M.Sc degree in Music and Acoustic Engineering from the Politecnico di Milano, Italy, in 2020. He is currently a Ph.D. student with the Image and Sound Processing Lab (ISPL) at the Department of Electronics, Information and Bioengineering (DEIB) of the Politecnico di Milano. His research activity focuses on signal processing for multimedia forensics applications. He is Co-Organizer of the IEEE Signal Processing Cup 2022.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/pbestagini.png}}]{Paolo Bestagini} (S’11-M'15) was born in Novara, Italy, in 1986. He received the M.Sc. degree in Telecommunications Engineering and the Ph.D. degree in Information Technology from the Politecnico di Milano, Italy, in 2010 and 2014, respectively. He is currently Assistant Professor with the Image and Sound Processing Lab (ISPL) at the Department of Electronics, Information and Bioengineering (DEIB) of the Politecnico di Milano. His research interests focus on multimedia forensics and acoustic signal processing for microphone arrays. He has been scientific investigator for the European projects SCENIC and REWIND coordinated by the Politecnico di Milano. He has been co-principal investigator for the DARPA-funded MediFor project. He is co-principal investigator for the DARPA-funded SemaFor project. He is an elected member of the IEEE Information Forensics and Security Technical Committee for the second time. He serves as an Associate Editor for the IEEE Transactions on Circuits and Systems for Video Technology (TCSVT) and the Elsevier Journal of Visual Communication and Image Representation (JVCI). He is Co-Organizer of the IEEE Signal Processing Cup 2018 and 2022.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/stubaro.jpg}}]{Stefano Tubaro} (SM’01) was born in Novara, Italy, in 1957. He received the M.Sc. degree in Electronic Engineering from the Politecnico di Milano, Milan, Italy, in 1982. He then joined the Department of Electronics, Information and Bioengineering (DEIB), Politecnico di Milano, first as a Researcher of the National Research Council, and then in 1991 as an Associate Professor. Since 2004, he has been appointed as a Full Professor of telecommunication with the Politecnico di Milano. His current research interests include advanced algorithms for video and sound processing. He coordinates the research activities of the Image and Sound Processing Lab (ISPL) at the Department of Electronics, Information and Bioengineering (DEIB), Politecnico di Milano. He had the role of a Project Coordinator of the European Project ORIGAMI: A new paradigm for high-quality mixing of real and virtual and of the research project ICT-FET-OPEN REWIND: REVerse engineering of audio-VIsual coNtent Data. This last project was aimed at synergistically combining principles of signal processing, machine learning, and information theory to answer relevant questions on the past history of such objects. He has authored more than 180 scientific publications on international journals and congresses and has coauthored more than 15 patents. In the past few years, he has focused his interest on the development of innovative techniques for image and video tampering detection and, in general, for the blind recovery of the processing history of multimedia objects.
He is a member the IEEE Multimedia Signal Processing Technical Committee and of the IEEE SPS Image Video and Multidimensional Signal Technical Committee. He was in the organization committee of a number of international conferences, including the IEEE MMSP 2004/2013, the IEEE ICIP 2005, the IEEE AVSS 2005/2009, the IEEE ICDSC 2009, the IEEE MMSP 2013, and the IEEE ICME 2015. From 2012 to 2015, he was an Associate Editor of the IEEE Transactions on Image Processing (TIP), and he is currently an Associate Editor of the IEEE Transactions on Information Forensics and Security (TIFS).
\end{IEEEbiography}

